Alpha-conversion for lambda terms with explicit weakenings

Using explicit weakenings, we can define alpha-conversion by simple equations without any mention of free variables.

==> section4.tex <==
\section{Free variables}
\begin{definition} Free variables.
In general case $FV(M)$ is a sequence\\
 $FV_0(M),FV_1(M), FV_2(M)\ldots$\\
 where each $FV_i(M)$ is a finite set of variables and\\
$FV(\x)=\{\x\},\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\up M)=\emptyset,FV_0(M),FV_1(M)\ldots$\\
$FV(MN)=FV_0(M)\cup FV_0(N),FV_1(M)\cup FV_1(N)\ldots$\\
$FV(\lambda\x M)=(FV_0(M)-\{\x\})\cup FV_1(M), FV_2(M), FV_3(M)\ldots$\\
The same definition more rigorously\\
$FV_0(\x)=\{\x\}$\\
$FV_{i+1}(\x)=\emptyset$\\
$FV_0(\up M)=\emptyset$\\
$FV_{i+1}(\up M)=FV_i(M)$\\
$FV_0(\lambda\x M)=(FV_0(M)-\{\x\})\cup FV_1(M)$\\
$FV_{i+1}(\lambda\x M)=FV_{i+2}(M)$

\end{definition}

\begin{example}$ $\\
$FV(x)=\{x\},\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\up x)=\emptyset,\{x\},\emptyset,\emptyset\ldots$\\
$FV(\lambda x\!\up x)=\{x\},\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\lambda x\lambda x\!\up x)=\emptyset,\emptyset,\emptyset\ldots$
\end{example}

\begin{definition} Free variables for de Bruijn's terms.\\
$FV(\x)=\{\x\},\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\un)=\emptyset,\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\up A)=\emptyset,FV_0(M),FV_1(M)\ldots$\\
$FV(AB)=FV_0(A)\cup FV_0(B),FV_1(A)\cup FV_1(B)\ldots$\\
$FV(\lambda A)=FV_0(A)\cup FV_1(A), FV_2(A), FV_3(A)\ldots$\\
The same definition more rigorously\\
$FV_0(\x)=\{\x\}$\\
$FV_{i+1}(\x)=\emptyset$\\
$FV_i(\un)=\emptyset$\\
$FV_0(\up A)=\emptyset$\\
$FV_{i+1}(\up A)=FV_i(A)$\\
$FV_0(\lambda A)=FV_0(A)\cup FV_1(A)$\\
$FV_{i+1}(\lambda A)=FV_{i+2}(A)$

\end{definition}

\begin{example}$ $\\
$FV(x)=\{x\},\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\up x)=\emptyset,\{x\},\emptyset,\emptyset\ldots$\\
$FV(\lambda \!\up x)=\{x\},\emptyset,\emptyset,\emptyset\ldots$\\
$FV(\lambda \lambda \!\up x)=\{x\},\emptyset,\emptyset\ldots$
\end{example}

\begin{theorem} $FV\|nil\vdash M\|=FV(M)$
\end{theorem}


